Chaff Bugs: Deterring Attackers by Making Software Buggier

Sophisticated attackers find bugs in software, evaluate their exploitability, and then create and launch exploits for bugs found to be exploitable. Most efforts to secure software attempt either to eliminate bugs or to add mitigations that make exploitation more difficult. In this paper, we introduce a new defensive technique called chaff bugs, which instead target the bug discovery and exploit creation stages of this process. Rather than eliminating bugs, we instead add large numbers of bugs that are provably (but not obviously) non-exploitable. Attackers who attempt to find and exploit bugs in software will, with high probability, find an intentionally placed non-exploitable bug and waste precious resources in trying to build a working exploit. We develop two strategies for ensuring non-exploitability and use them to automatically add thousands of non-exploitable bugs to real-world software such as nginx and libFLAC; we show that the functionality of the software is not harmed and demonstrate that our bugs look exploitable to current triage tools. We believe that chaff bugs can serve as an effective deterrent against both human attackers and automated Cyber Reasoning Systems (CRSes).

==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

The bugs we can inject are highly related to the coverage from the inputs.
However, there still would be a certain part of the code can never be covered in our bug injection because of the limited attacking surface. It's not necessarily a problem that we can't put bugs into parts of the program that are not affected by the input, because those parts of the program wouldn't contain exploitable bugs anyway. In our Nginx experiment, we failed to touch some parts of the code that is too fundamental like code implementing spin locks, and system log modules because it is not directly related to the attacker's input, while on the other hand we managed to insert code into other basic modules including nginx format string module, memory management module because they are highly related to the input.

%bugs are selected randomly, however, there are more overconstraint bugs because of the attack point selection. Sometimes we may not even get unused type bugs at all if selected randomly. N overconstraint bugs, and M unused bugs. To compensentate this, we intentionally add a extra unused bugs at a 
%For the number of different type of bugs, we are expecting different number in total because of the limited attack point selection strategy for unused bugs. As a result, we are expecting more overconstraint bugs than unused bugs. As a result, we got \fxwarning{N} overconstraint bugs and \fxwarning{M} unused bugs. Which random selection may not get all the bugs selected evenly. Sometimes we ended up with only overconstraint bugs injected. This did not have any impact on our evaluations.

%While in the use of DUA, we also encountered a few partially initialized variables, which only a part of the structure is initialized while we are referencing the uninitialized filed of that variable. The consequence is that we may crash on the original input when referencing this uninitialized value. Our current solution is to remove it at the stage of bug validation when it crashes. However, this relies heavily on the validation inputs to perform a thorough test. Another approach is to enforce a stricter rule in defining variable initialization. Since this problem only exists when the structured object is initialized through function arguments, we could simply discard this situation as a valid initialization. The cost will be that we may lose even more bugs being able to triggered.
%\begin{lstlisting}
%void
%ngx_reusable_connection(ngx_connection_t *c, ngx_uint_t reusable)
%{
%  ...
%  lava_set(((*c).buffer).start);
%  ...
%}
%\end{lstlisting}

While in the libFLAC experiment, we have to patch the integrity checks to get enough valid DUAs. As we have noted in the evaluation, the high TCN value caused by the integrity checks violates our basic assumption of "Uncomplicated" data. But in fact, the checked data may not be really so complicated, it is only the CRC calculation makes the TCN goes really high. In deploy, we rely on the developer to disable the integrity checks. For performance concern, we tend to keep the media corpus small, which might limit us to find more usable DUAs. For our current workbench, we do not have enough computing power for a large scale taint analysis that could process the lossless media files of normal size.

%\begin{listing}
%\centering
%\begin{minted}{c}
%for(channel = 0; channel < decoder->private_->frame.header.channels; channel++)
%{
%	/* Do Something */
%}
%\end{minted}
%\caption{Variable TCN}
%\label{lst:patchmisbehave}
%\end{listing}




==> secproof.tex <==

% All the extra codes Injected
%%
%Setting the trigger
%%
%if (lava\_hits(DUA) == N)
%	lava\_set(hash(id), *(uint32\_t *)((*((*a).member)).member + offset);									<===== OOB Read
%																											
%																											struct Foo* foo = param->foo;
%																											lava\_set(foo->begin\_ptr);
%																											
%																											visited multiple times and begin\_ptr reaches the end, OOB!

%%
%Unused bug
%%
%if (lava\_get(hash(id)) == Trigger) {
%	memcpy(&(DUA2) + sizeof(DUA2), DUA3, 4);								<=== I think this is safe, because Struct Objects are skipped;
%	*lava\_data\_flow = *lava\_padding\_##DUA2;									 If DUA3 got an OOB Read, it's still alright
%}

%%FP rootFunc(args...) {
%	int lava\_data\_flow[1];
%	funcCall(lava\_data\_flow, ...);
%	(a->funcPtr == fp1 || a->funcPtr == fp2) ? a->funcPtr(lava\_data\_flow, ...) : a->funcPtr(...);
%}

%%
%Overconstraint bug
%%
%if (lava\_get(hash(id)) == Trigger && !isSafeValue(DUA2))
%	abort();


%if (lava\_get(hash(id)) == Trigger)
%	memcpy(lava\_var\_at\_stack\_base + jumpoffset, DUA2, 4);					<=== DUA2 is where bothers me
%																					 (Solution?) Maybe zero out the stored trigger once reached there? Since our bug should be pretty shallow.
																					 
																					 
																					 
																					 




\subsection{Trigger Time}


%bugs -- stack  - unused			v(2 unused var)
%	  |		   - overconstraint
%	  |
%	  - heap   - unused			v(add it)
%			   - overconstraint
			   
			   


